Less is More: Learning Prominent and Diverse Topics for Data Summarization

Statistical topic models efficiently facilitate the exploration of large-scale data sets. Many models have been developed and broadly used to summarize the semantic structure in news, science, social media, and digital humanities. However, a common and practical objective in data exploration tasks is not to enumerate all existing topics, but to quickly extract representative ones that broadly cover the content of the corpus, i.e., a few topics that serve as a good summary of the data. Most existing topic models fit exactly the same number of topics as a user specifies, which have imposed an unnecessary burden to the users who have limited prior knowledge. We instead propose new models that are able to learn fewer but more representative topics for the purpose of data summarization. We propose a reinforced random walk that allows prominent topics to absorb tokens from similar and smaller topics, thus enhances the diversity among the top topics extracted. With this reinforced random walk as a general process embedded in classical topic models, we obtain \textit{diverse topic models} that are able to extract the most prominent and diverse topics from data. The inference procedures of these diverse topic models remain as simple and efficient as the classical models. Experimental results demonstrate that the diverse topic models not only discover topics that better summarize the data, but also require minimal prior knowledge of the users.

==> introduction__Jian_Tang_s_conflicted_copy_2013-08-14_.tex <==
\section{Introduction}
The online information is now increasing at unprecedented speed. A hug amount of data, known as ``big data'',  is generated from social media websites such as Twitter, Facebook, Google++, search engine log,  and so on. To facilitate the exploration and retrieval of the big data, it is becoming increasingly important to develop tools to understand and summarize the data automatically. 

Statistical topic models, e.g., probabilistic latent semantic analysis (PLSA)~\cite{hofmann1999probabilistic} and latent Dirichlet allocation (LDA)~\cite{blei2003latent}, are the tools to help users to understand and summarize the data. The models are able to automatically infer the hidden themes (a.k.a.\ topics) pervading the data and meanwhile annotate the data according to these themes. With these annotations, it becomes much easier for users to explore and search the entire data.

Given a new data collection, a common question users would ask is: ``what are the most important aspects in the data?'' Therefore, in order to give a good summarization of the data, it would be desirable to discover the most important topics within the data. One straightforward way is to deploy the off-the-shelf topic models, e.g., LDA,  to train a few topics on the entire dataset, which users would expect to be the most important topics in the data. However, fitting only a few topics to a big collection of data is quite likely to under-fit the data. Each of the inferred topics are likely to be a mixture of multiple topics, which cannot be interpreted by users at all and hence cannot convey any useful information at all.
	
\begin{figure*}[htdb!]
\centering
\subfigure[\small Topic Network with PLSA]{
\includegraphics[width=1.5in]{/Users/Jian/Experiment/WSDM2014/animation/4conf/result/divplsa_topic_network_plsa.pdf}
\label{fig:network-plsa}
}
\subfigure[\small Topic Network with DivPLSA]{
\includegraphics[width=1.5in]{/Users/Jian/Experiment/WSDM2014/animation/4conf/result/divplsa_topic_network_divplsa.pdf}
\label{fig:network-divplsa}
}
\subfigure[\small Topics by PLSA and DivPLSA]{
\scalebox{0.67}{
\begin{tabular}{c|c|c|c|c|c} \hline
\multicolumn{3}{c}{PLSA} & \multicolumn{3}{c}{DivPLSA} \\ \hline
ID&Proportion&Top Words & ID&Proportion&Top Words \\ \hline
17&8.13\%&retrieval information system document model systems based & 16&27.58\%&learning classification models clustering algorithm support bayesian  \\\hline
0&7.17\%&data mining large databases patterns discovery sets & 17&24.39\%&retrieval information text query system document evaluation \\\hline
14&6.55\%&learning reinforcement control function training optimal active  &15&21.77\%&neural networks network model recognition visual learning \\ \hline
16&6.49\%&clustering models gaussian probabilistic regression study inference  &11&17.11\%&web search semantic xml extraction analysis content \\ \hline
15&6.14\%&visual model human models computer motion maps  &0&15.03\%&data mining knowledge discovery large databases rules \\ \hline
%11&6.05\%&web documents xml search extraction browsing pages  &&&\\ \hline
%9&5.54\%&classification support image vector feature filtering machine  &&&\\ \hline
%6&5.47\%&network neural recognition speech modeling estimation adaptive  &&&\\ \hline
%7&5.11\%&networks neural neurons video associative artificial statistical  &&&\\ \hline
%4&5.04\%&text automatic search similarity categorization topic statistical  &&&\\ \hline
\end{tabular}
}
\label{fig:intro-topics-comparsion}
}
\label{motivation}
\caption{An example to compare the topics inferred by classical topic models and our diverse topic models.}
\end{figure*}

As it is generally difficult to estimate an appropriate number of topics in the data, an alternative way is to fit a large number of topics to the data and pick the most important topics, e.g., the topics with the largest size, which would be generally meaningful to users. However, fitting too many topics to the data would over-fit the data and the inferred topics tend to be small and duplicated with each other. 
%%%%%%%%modify this
This would not be a good summarization of the data as the selected topics in this way will have a low information coverage.  To give a good summarization, the selected topics should be important, i.e., having a high information coverage, and meanwhile non-redundant. 
This motivates us to learn the most prominent and diverse topics pervading the data. 

An intuitive way to achieve this is to automatically merge the similar topics in the over-fitting case. Once the similar topics are merged, we are likely to obtain large and diverse topics. We give a motivating example below.

\noindent\textbf{Example.} We collected the metadata of papers from four conferences including ``SIGIR'', ``KDD'', ``WWW'' and ``NIPS''. Each author is treated as a document by aggregating the titles of his papers. Figure \ref{fig:network-plsa} shows the topic networks generated by training PLSA with 20 topics, and the left part of Figure \ref{fig:intro-topics-comparsion} shows the largest five topics. We can see that the selected topics through this way is small and similar. Figure \ref{fig:network-divplsa} shows the topic network after the similar topics are merged and the right part of Figure \ref{fig:intro-topics-comparsion} shows the corresponding topics. Five topics including ``learning'', ``information retrieval'', ``neural network'', ``Web'', and ``data mining'' are finally kept. Considering that the data are collected from the four conferences aforementioned, the discovered topics well summarize the original data.

In this paper, we proposed a \emph{topic size-reinforced random walk} to automatically merge similar topics. Specifically, during the learning process of topic models, the network among the topics is built to model the relationships among the topics. For each token in the data, after assigning it to one topic in the network, we further allow it to transit to other topics in the network, including the topic itself. The transition probability is determined by the similarity among the topics and \emph{reinforced} by the size of the topic, i.e., the number of tokens assigned to it.  During this process, we can see that all the topics are competing resources, i.e., word tokens,  from each other. The tokens belonging to the smaller topics are likely to transit to the larger similar topics. In other words, the larger topics will \emph{absorb} the smaller topics.  This will result the \emph{rich-gets-richer} phenomenon, i.e., the larger topics become larger by absorbing tokens from smaller similar topics. The whole process converges until all the smaller similar topics are absorbed and end up with larger and diverse topics, which cannot be absorbed by each other. 

We embed the \emph{topic size-reinforced random walk} process into the off-the-shelf topic models PLSA and LDA, and obtained two diverse topic models DivPLSA (abbreviation for diverse PLSA) and DivLSA( abbreviation for diverse LDA). The learning procedures of the two models remain as simple and efficient as the classical ones but able to learn the prominent and diverse topics pervading the data. We evaluate the effectiveness of the two diverse topic models on four real-world datasets. Experimental results show that the proposed models discover better topics for data summarization than classical topic models.

\noindent{\textbf{Organization.}} The rest of this paper is organized as follows. Section 2 discusses the related work. Section 3 formally defines the problem of applying topic modeling for data summarization. Section 4 introduces the topic size-reinforced random walk and two diverse topic models DivPLSA and DivLDA. The effectiveness of the two models are empirically evaluated in Section 5. Finally in Section 6 we conclude this paper and point out the future work. 
